Learning to Benchmark: Determining Best Achievable Misclassification Error from Training Data

We address the problem of learning to benchmark the best achievable classifier performance. In this problem the objective is to establish statistically consistent estimates of the Bayes misclassification error rate without having to learn a Bayes-optimal classifier. Our learning to benchmark framework improves on previous work on learning bounds on Bayes misclassification rate since it learns the {\it exact} Bayes error rate instead of a bound on error rate. We propose a benchmark learner based on an ensemble of $\epsilon$-ball estimators and Chebyshev approximation. Under a smoothness assumption on the class densities we show that our estimator achieves an optimal (parametric) mean squared error (MSE) rate of $O(N^{-1})$, where $N$ is the number of samples. Experiments on both simulated and real datasets establish that our proposed benchmark learning algorithm produces estimates of the Bayes error that are more accurate than previous approaches for learning bounds on Bayes error probability.

==> feature_selection.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Bayes Error Based Feature Selection}\label{sec:BEFS}

In this section we show that Bayes error estimates can be used for feature selection. The problem is, given a set of initial features, choose a smaller set of features that can provide the maxumum distinguishability between different classes.
Assume that the input data denoted by a random variable $X$ consists of $d$ features as $X=[X^1,...,X^d]$ and we are asked to select  a set of $r$ features ($r<d$). Our proposed forward selection method consists of $r$ steps, where at each step we choose a feature from $\{X^1,...,X^d\}$ that reduces the Bayes error the most. The advantage of this feature selection method is that it does not depend on any specific model. The pseudocode for the proposed Bayes error based feature selection (BEFS) method is given in Algorithm \ref{algo:feature_selection}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm} 
\DontPrintSemicolon
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% Input:
\Input{
Input dataset, $\bX=\{X_1,...,X_N\}$\\
Labels, $\bY=\{Y_1,...,Y_N\}$\\
Desired number of output features, $r$}

\BlankLine

$\mathcal{F}:=\phi$

\For {each $i\in \{1,...,r\}$}{

         $f \leftarrow \argmax \{BER\{\mathcal{F}\} - BER\{\mathcal{F}\cup X^j\}$ \\ 
		 Add $f$ into $\mathcal{F}$
		 
		 }

\Output{$\mathcal{F}$}

\caption{Bayes Error Based Feature Selection (BEFS)}
\label{algo:feature_selection}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We apply BEFS method on two real-datasets: breast cancer Wisconsin (diagnostic) dataset \citep{wolberg1995image} and robot navigation dataset (both downloaded from UC Irvine Machine Learning Repository)

In the breast cancer dataset, there are 9 features, generated from image analysis of fine needle aspirates (FNA) of breast masses and characterise cell nucleus properties, and the task to classify the patients into the classes \textit{malignant} or
\textit{benign breast mass}. The set of measured features are Clump thickness,
uniformity of cell size,
uniformity of cell shape,
marginal adhesion,
single epithelial cell size,
number of bare nuclei,
bland chromatin,
number of normal nuclei, and 
Mitosis. Each of the features is a real value in the range $[0,1]$. We apply BEFS on this dataset to get the first $5$ most important features for the diagnosis. Figure \ref{fig:BC} represents the order of the selected first $5$ features with the respective Bayes error of the selected feature set. The selected features are uniformity of cell shape, bare nuclei, marginal adhesion , clump thickness, bland chromatin (in the order of importance). 

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\textwidth]{fig/BC.png}
	%\vspace{-0.5cm}
	\caption{Order of the selected variables: 
    uniformity of cell shape, bare nuclei, marginal adhesion , clump thickness, bland chromatin 
}\label{fig:BC}
\end{figure}

%%%%%%%%%%%%%



%%%%%%%%%%%%
The second dataset is the wall-following robot navigation data \citep{freire2009short}.
The data are measurements of the $24$ ultrasound sensors arranged circularly around a robot (Figure \ref{fig:sensor_selection_robot}). The task for the robot is to navigate in a clockwise direction around the room, by following the wall. The dataset consists of 5456 recorded timestamps. 
At each timestamp, the robot gets the measurements from all of the sensors and decides which action should it take. The possible actions include one of the four classes move-forward, sharp-right-turn, slight-right-turn and turn-left. We apply the proposed feature selection method on this dataset. According to Figure \ref{fig:feature_selection_robot}, the selected sensors are $S_{15},S_{18},S_{12},S_{20},S_{19}$ (in the order of importance).


\begin{figure}[!h]
	\centering
	\includegraphics[width=0.95\textwidth]{fig/robot.png}
	%\vspace{-0.5cm}
	\caption{The graphs of the SCITOS G5 robot with $24$ ultrasound sensors arranged circularly around a robot (left), the followed path by the robot (middle), and the positions and the indexing of the sensors $1$ through $24$ (right). The task for the robot is to navigate in a clockwise direction around the room, by following the wall. The dataset consists of 5456 recorded timestamps. At each timestamp, the robot gets the measurements from all of the sensors and decides which action should it take. The possible actions include one of the four directions: move-forward, sharp-right-turn, slight-right-turn and turn-left.}\label{fig:sensor_selection_robot}
\end{figure}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.8\textwidth]{fig/sensor_selection_robot.png}
	%\vspace{-0.5cm}
	\caption{Order of the selected sensors using BEFS method for the robot navigation dataset. The selected sensors are $S_{15},S_{18},S_{12},S_{20},S_{19}$ (in the order of importance).}\label{fig:feature_selection_robot}
\end{figure}


